Asymptotic behaviour of rescaled nonlocal functionals and evolutions

Taking up a variational viewpoint, we present some nonlocal-to-local asymptotic results for various kinds of integral functionals. The content of the thesis comprises the contributions first appeared in some research papers in collaboration with J. Berendsen, A. Cesaroni, A. Chambolle, and M. Novaga.

==> cap4.5-clusters.tex <==
\begin{rmk}[Outlook]
			see the analysis carried out in \cite{AB2} for ``localised'' functionals.
			
			The cases when $K$ changes sign or when it is substituted by a Radon measure $\mu$
			are also possible subjects of further study,
			but the conclusions of Theorem \ref{stm:Gammaconv} might be affected.
			
			Finally, it would be interesting to obtain a $\Gamma$-convergence result for multi-phase systems,
			i.e. for functionals of the form
			\[J_\eps(E_1,\dots,E_N) \sum_{0\leq i<j\leq N} a_{i,j}L_\eps(E_i,E_j),\]
			where $E_1,\dots,E_N$ are measurable sets such that $\va{E_i}>0$ and $\va{E_i\cap E_i}=0$ for any $i,j=1,\dots,N$,
			$E_0  \coloneqq \co{(\bigcup_{i=1}^N E_i)}$ and
			the coefficients $a_{i,j}$ are positive and they satisfy $a_{i,j}\leq a_{i,k}+a_{k,j}$
			for every $i,j,k=0,\dots,N$. 
			As a particular instance,
			if for any $i=0,\dots,N$ there exists $a_i\geq0$ such that
			$a_i=a_{i,j}$ for all $j\neq i$, we get
			\[J_\eps(E_1,\dots,E_N)= \frac{1}{2}\sum_{i=0}^N a_{i}J_\epsilon(E_i,\Rd);\]
			in this case, it easy to recover a $\Gamma$-convergence result from the theory we developed in this paper.
		\end{rmk}
